Learning to Communicate with Strangers via Channel Randomisation Methods

We introduce two methods for improving the performance of agents meeting for the first time to accomplish a communicative task. The methods are: (1) `message mutation' during the generation of the communication protocol; and (2) random permutations of the communication channel. These proposals are tested using a simple two-player game involving a `teacher' who generates a communication protocol and sends a message, and a `student' who interprets the message. After training multiple agents via self-play we analyse the performance of these agents when they are matched with a stranger, i.e. their zero-shot communication performance. We find that both message mutation and channel permutation positively influence performance, and we discuss their effects.

==> figures/causal-diagram.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,387); %set diagram left start at 0, and has height of 387

%Shape: Trapezoid [id:dp5901240262993543] 
\draw   (30,100) -- (49.88,140) -- (70.12,140) -- (90,100) -- cycle ;
%Straight Lines [id:da6011527928496057] 
\draw    (60,80) -- (60,98) ;
\draw [shift={(60,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3025827846535829] 
\draw    (80,120) -- (148,120) ;
\draw [shift={(150,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Trapezoid [id:dp9819832748620978] 
% \draw   (90,240) -- (70.12,200) -- (49.88,200) -- (30,240) -- cycle ;
% %Straight Lines [id:da1790721168726228] 
% \draw    (60,260) -- (60,242) ;
% \draw [shift={(60,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp3862968733798853] 
\draw   (90,150) -- (130,150) -- (130,190) -- (90,190) -- cycle ;
% %Straight Lines [id:da053951695704332] 
% \draw    (60,170) -- (60,200) ;
% %Straight Lines [id:da37287004413016644] 
% \draw    (60,170) -- (88,170) ;
% \draw [shift={(90,170)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da19801026797825405] 
\draw    (110,80) -- (110,150) ;
%Straight Lines [id:da31221967512904425] 
\draw    (160,80) -- (160,98) ;
\draw [shift={(160,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da542187448390171] 
\draw    (110,80) -- (160,80) ;

% %Straight Lines [id:da94636452801409] 
% \draw    (80,220) -- (148,220) ;
% \draw [shift={(150,220)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Trapezoid [id:dp28862182434576344] 
\draw   (140,100) -- (159.88,140) -- (180.12,140) -- (200,100) -- cycle ;
%Straight Lines [id:da7711829868040181] 
\draw    (190,120) -- (258,120) ;
\draw [shift={(260,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Trapezoid [id:dp17079176405149266] 
% \draw   (200,240) -- (180.12,200) -- (159.88,200) -- (140,240) -- cycle ;
% %Straight Lines [id:da5849552322493206] 
% \draw    (180,260) -- (180,242) ;
% \draw [shift={(180,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp7430365274815369] 
\draw   (200,150) -- (240,150) -- (240,190) -- (200,190) -- cycle ;
% %Straight Lines [id:da12259814895667787] 
% \draw    (170,170) -- (170,200) ;
% %Straight Lines [id:da5277029726961073] 
% \draw    (170,170) -- (198,170) ;
% \draw [shift={(200,170)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da12648955985829313] 
\draw    (220,80) -- (220,150) ;
%Straight Lines [id:da6717632559091897] 
\draw    (270,80) -- (270,98) ;
\draw [shift={(270,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7852237534773034] 
\draw    (220,80) -- (270,80) ;

% %Straight Lines [id:da025396926289187993] 
% \draw    (190,220) -- (258,220) ;
% \draw [shift={(260,220)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9942191441072064] 
\draw    (179,80) -- (179,98) ;
\draw [shift={(179,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Trapezoid [id:dp22639767383286324] 
\draw   (250,100) -- (269.88,140) -- (290.12,140) -- (310,100) -- cycle ;
%Straight Lines [id:da8492176559468829] 
\draw    (300,120) -- (368,120) ;
\draw [shift={(370,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Trapezoid [id:dp5472863558493164] 
% \draw   (310,240) -- (290.12,200) -- (269.88,200) -- (250,240) -- cycle ;
% %Straight Lines [id:da3912463612280437] 
% \draw    (290,260) -- (290,242) ;
% \draw [shift={(290,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Rectangle [id:dp44843731628943706] 
% \draw   (310,150) -- (350,150) -- (350,190) -- (310,190) -- cycle ;
% %Straight Lines [id:da7111784114961179] 
% \draw    (280,170) -- (280,200) ;
% %Straight Lines [id:da9629886535388228] 
% \draw    (280,170) -- (308,170) ;
% \draw [shift={(310,170)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% %Straight Lines [id:da7306046311155834] 
% \draw    (330,80) -- (330,150) ;
% %Straight Lines [id:da354384477381136] 
% \draw    (380,80) -- (380,98) ;
% \draw [shift={(380,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da7295669743116457] 
% \draw    (330,80) -- (380,80) ;

% %Straight Lines [id:da19180832123356528] 
% \draw    (300,220) -- (368,220) ;
% \draw [shift={(370,220)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da41479953685035587] 
\draw    (289,80) -- (289,98) ;
\draw [shift={(289,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Trapezoid [id:dp23778473396607813] 
% \draw   (360,100) -- (379.88,140) -- (400.12,140) -- (420,100) -- cycle ;
% %Straight Lines [id:da4969430231085945] 
% \draw    (410,120) -- (478,120) ;
% \draw [shift={(480,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Trapezoid [id:dp08174446763694543] 
% \draw   (420,240) -- (400.12,200) -- (379.88,200) -- (360,240) -- cycle ;
% %Straight Lines [id:da46063172456810353] 
% \draw    (400,260) -- (400,242) ;
% \draw [shift={(400,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Rectangle [id:dp49449743126583234] 
% \draw   (420,150) -- (460,150) -- (460,190) -- (420,190) -- cycle ;
% %Straight Lines [id:da06459758020868067] 
% \draw    (390,170) -- (390,200) ;
% %Straight Lines [id:da33220485232796304] 
% \draw    (390,170) -- (418,170) ;
% \draw [shift={(420,170)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% %Straight Lines [id:da6214791477895552] 
% \draw    (440,80) -- (440,150) ;
% %Straight Lines [id:da3841472585609973] 
% \draw    (490,80) -- (490,98) ;
% \draw [shift={(490,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da1908780101569454] 
% \draw    (440,80) -- (490,80) ;

% %Shape: Trapezoid [id:dp3159737818034316] 
% \draw   (470,100) -- (489.88,140) -- (510.12,140) -- (530,100) -- cycle ;
% %Straight Lines [id:da1828263964084922] 
% \draw    (500,140) -- (500,208) ;
% \draw [shift={(500,210)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da9435490721048199] 
% \draw    (110,260) -- (110,190) ;
% %Straight Lines [id:da9978288669432911] 
% \draw    (160,260) -- (160,242) ;
% \draw [shift={(160,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da008558160066979958] 
% \draw    (110,260) -- (160,260) ;

% %Straight Lines [id:da7693291904524184] 
% \draw    (220,260) -- (220,190) ;
% %Straight Lines [id:da35557035985411867] 
% \draw    (270,260) -- (270,242) ;
% \draw [shift={(270,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da6289233262454783] 
% \draw    (220,260) -- (270,260) ;

% %Straight Lines [id:da4697797774520691] 
% \draw    (330,260) -- (330,190) ;
% %Straight Lines [id:da1190721808374664] 
% \draw    (380,260) -- (380,242) ;
% \draw [shift={(380,240)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da3824169672422528] 
% \draw    (330,260) -- (380,260) ;


% % Text Node
% \draw (52,263.4) node [anchor=north west][inner sep=0.75pt]    {$o_{1}$};
% Text Node
\draw (52,63.4) node [anchor=north west][inner sep=0.75pt]    {$o_{t}$};
% Text Node
\draw (54,113) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t}$ };
% % Text Node
% \draw (54,216) node [anchor=north west][inner sep=0.75pt]   [align=left] {T};
% Text Node
\draw (103,165) node [anchor=north west][inner sep=0.75pt]   [align=left] { $m_t$ };
% Text Node
\draw (213,165) node [anchor=north west][inner sep=0.75pt]   [align=left] { $m_{t+1}$ };
% % Text Node
% \draw (173,263.4) node [anchor=north west][inner sep=0.75pt]    {$o_{2}$};
% % Text Node
% \draw (164,216) node [anchor=north west][inner sep=0.75pt]   [align=left] {T};
% Text Node
\draw (164,113) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t+1}$ };
% Text Node
\draw (171,63.4) node [anchor=north west][inner sep=0.75pt]    {$o_{t+1}$};
% % Text Node
% \draw (282,263.4) node [anchor=north west][inner sep=0.75pt]    {$o_{3}$};
% % Text Node
% \draw (274,216) node [anchor=north west][inner sep=0.75pt]   [align=left] {T};
% % Text Node
% \draw (323,165) node [anchor=north west][inner sep=0.75pt]   [align=left] {m};
% Text Node
\draw (281,63.4) node [anchor=north west][inner sep=0.75pt]    {$o_{t+2}$};
% Text Node
\draw (274,113) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t+2}$ };
% % Text Node
% \draw (392,263.4) node [anchor=north west][inner sep=0.75pt]    {$o_{f}$};
% % Text Node
% \draw (384,216) node [anchor=north west][inner sep=0.75pt]   [align=left] {T};
% Text Node
% \draw (433,165) node [anchor=north west][inner sep=0.75pt]   [align=left] {m};
% Text Node
\draw (384,113) node [anchor=north west][inner sep=0.75pt]   [align=left] {I};
% % Text Node
% \draw (494,113) node [anchor=north west][inner sep=0.75pt]   [align=left] {S};
% % Text Node
% \draw (495,212.4) node [anchor=north west][inner sep=0.75pt]    {$\hat{y}_f$};


\end{tikzpicture}


==> figures/causal-matcha-diagram.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,387); %set diagram left start at 0, and has height of 387

%Straight Lines [id:da11436674693328652] 
\draw    (60,80) -- (60,98) ;
\draw [shift={(60,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da26622416120838943] 
\draw    (80,120) -- (148,120) ;
\draw [shift={(150,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da12428272859018008] 
\draw    (190,120) -- (258,120) ;
\draw [shift={(260,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4877507635946976] 
\draw    (300,120) -- (368,120) ;
\draw [shift={(370,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Connector [id:dp9392485248091521] 
\draw   (40.2,119.87) .. controls (40.01,109.09) and (48.87,100.19) .. (60,100) .. controls (71.13,99.81) and (80.3,108.39) .. (80.49,119.17) .. controls (80.67,129.95) and (71.81,138.85) .. (60.68,139.04) .. controls (49.56,139.23) and (40.38,130.65) .. (40.2,119.87) -- cycle ;
%Flowchart: Connector [id:dp4563717004309392] 
\draw   (149.71,120.7) .. controls (149.52,109.92) and (158.39,101.03) .. (169.51,100.83) .. controls (180.64,100.64) and (189.81,109.22) .. (190,120) .. controls (190.19,130.78) and (181.32,139.68) .. (170.2,139.87) .. controls (159.07,140.07) and (149.9,131.48) .. (149.71,120.7) -- cycle ;
%Flowchart: Connector [id:dp9751911384112375] 
\draw   (259.71,120.7) .. controls (259.52,109.92) and (268.39,101.03) .. (279.51,100.83) .. controls (290.64,100.64) and (299.81,109.22) .. (300,120) .. controls (300.19,130.78) and (291.32,139.68) .. (280.2,139.87) .. controls (269.07,140.07) and (259.9,131.48) .. (259.71,120.7) -- cycle ;
%Flowchart: Connector [id:dp0023080831159817405] 
\draw   (370,120) .. controls (369.81,109.22) and (378.68,100.32) .. (389.8,100.13) .. controls (400.93,99.93) and (410.1,108.52) .. (410.29,119.3) .. controls (410.48,130.08) and (401.61,138.97) .. (390.49,139.17) .. controls (379.36,139.36) and (370.19,130.78) .. (370,120) -- cycle ;
%Flowchart: Connector [id:dp8761547274915173] 
\draw   (39.51,60.83) .. controls (39.33,50.05) and (48.19,41.15) .. (59.32,40.96) .. controls (70.44,40.77) and (79.62,49.35) .. (79.8,60.13) .. controls (79.99,70.91) and (71.13,79.81) .. (60,80) .. controls (48.87,80.19) and (39.7,71.61) .. (39.51,60.83) -- cycle ;
%Flowchart: Connector [id:dp6665722885558577] 
\draw   (158.51,60.83) .. controls (158.33,50.05) and (167.19,41.15) .. (178.32,40.96) .. controls (189.44,40.77) and (198.62,49.35) .. (198.8,60.13) .. controls (198.99,70.91) and (190.13,79.81) .. (179,80) .. controls (167.87,80.19) and (158.7,71.61) .. (158.51,60.83) -- cycle ;
%Flowchart: Connector [id:dp2205456371639557] 
\draw   (268.51,60.83) .. controls (268.33,50.05) and (277.19,41.15) .. (288.32,40.96) .. controls (299.44,40.77) and (308.62,49.35) .. (308.8,60.13) .. controls (308.99,70.91) and (300.13,79.81) .. (289,80) .. controls (277.87,80.19) and (268.7,71.61) .. (268.51,60.83) -- cycle ;
%Straight Lines [id:da3217866805495764] 
\draw    (179,80) -- (179,102) ;
\draw [shift={(179,104)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21603050453078854] 
\draw    (160,80) -- (160,102) ;
\draw [shift={(160,104)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8448064020287113] 
\draw    (110,80) -- (110,150) ;
%Straight Lines [id:da34966925481707367] 
\draw    (110,80) -- (160,80) ;

%Straight Lines [id:da136354385655302] 
\draw    (270,80) -- (270,102) ;
\draw [shift={(270,104)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da06770279917879418] 
\draw    (220,80) -- (220,150) ;
%Straight Lines [id:da3171196126291401] 
\draw    (220,80) -- (270,80) ;

%Straight Lines [id:da47333059876385364] 
\draw    (289,80) -- (289,102) ;
\draw [shift={(289,104)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Connector [id:dp9552502761968278] 
\draw   (90.2,169.87) .. controls (90.01,159.09) and (98.87,150.19) .. (110,150) .. controls (121.13,149.81) and (130.3,158.39) .. (130.49,169.17) .. controls (130.67,179.95) and (121.81,188.85) .. (110.68,189.04) .. controls (99.56,189.23) and (90.38,180.65) .. (90.2,169.87) -- cycle ;
%Flowchart: Connector [id:dp4644867940880836] 
\draw   (200.34,169.52) .. controls (200.15,158.74) and (209.02,149.84) .. (220.14,149.65) .. controls (231.27,149.45) and (240.44,158.04) .. (240.63,168.82) .. controls (240.82,179.6) and (231.95,188.49) .. (220.83,188.69) .. controls (209.7,188.88) and (200.53,180.3) .. (200.34,169.52) -- cycle ;

% Text Node
\draw (54,55) node [anchor=north west][inner sep=0.75pt]    {$o_{t}$};
% Text Node
\draw (55,114) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t}$ };
% Text Node
\draw (104,164) node [anchor=north west][inner sep=0.75pt]   [align=left] { $m_t$ };
% Text Node
\draw (215,164) node [anchor=north west][inner sep=0.75pt]   [align=left] { $m_{t+1}$ };
% Text Node
\draw (165,114) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t+1}$ };
% Text Node
\draw (172,55) node [anchor=north west][inner sep=0.75pt]    {$o_{t+1}$};
% Text Node
\draw (283,55) node [anchor=north west][inner sep=0.75pt]    {$o_{t+2}$};
% Text Node
\draw (274.03,114) node [anchor=north west][inner sep=0.75pt]   [align=left] { $Z_{t+2}$ };
% Text Node
\draw (385,114) node [anchor=north west][inner sep=0.75pt]   [align=left] {I};

\end{tikzpicture}
